Global simulations of Tayler instability in stellar interiors: a long-time multi-stage evolution of the magnetic field

Magnetic fields have been observed in massive Ap/Bp stars and presumably are also present in the radiative zone of solar-like stars. Yet, to date there is no clear understanding of the dynamics of the magnetic field in stably stratified layers. A purely toroidal magnetic field configuration is known to be unstable, developing mainly non-axisymmetric modes. Rotation and a small poloidal field component may lead to a stable configuration. Here we perform global MHD simulations with the EULAG-MHD code to explore the evolution of a toroidal magnetic field located in a layer whose stratification resembles the solar tachocline. Our numerical experiments allow us to explore the initial unstable phase as well as the long-term evolution of the magnetic field. During the first Alfven cycles, we observe the development of the Tayler instability with the prominent longitudinal wavenumber, $m=1$. Rotation decreases the growth rate of the instability, and eventually suppresses it. However, after a stable phase, sudden energy surges lead to the development of higher order modes even for fast rotation. These modes extract energy from the initial toroidal field. Nevertheless, our results show that sufficiently fast rotation leads to a lower saturation energy of the unstable modes, resulting in a magnetic topology with only a small fraction of poloidal field which remains steady for several hundreds of Alfven travel times. At this stage, the system becomes turbulent and the field is prone to turbulent diffusion. The final toroidal-poloidal configuration of the magnetic field may represent an important aspect of the field generation and evolution in stably-stratified layers.

==> referee.tex <==
% \input{preamble.tex} %Importando o preâmbulo

% % ---------------------------------------------------------- 
% % CONFIGURAÇÕES PESSOAIS
% % ----------------------------------------------------------	
% \newcommand{\soptitle}{Answer To Referee}
% \newcommand{\yourname}{Guilherme Monteiro}
% \newcommand{\youremail}{guiaudias@ufmg.br}

% % ----------------------------------------------------------
% \begin{document} 
% % ----------------------------------------------------------
% %Making my own title
% \begin{center}\LARGE\soptitle\\
% \large \yourname\\\youremail\\ 
% \end{center}
% \hrule
% \vspace{0.1cm}
% \hrule height 0.1cm
% \vspace{0.3cm}
% % ----------------------------------------------------------

% \section*{Comments to the Author}

% The paper “Global simulations of Tayler instability in stellar interiors: a long-time multi-stage evolution of the magnetic field” by Guilherme Monteiro et al. studies Tayler instability of toroidal magnetic fields in stably stratified stellar interiors by 3D direct numerical simulations (DNS). The computations reproduce the formerly known initial exponential growth of the instability and discover new essentially nonlinear stages of saturation and eventual decay in the instability development. These are significant new results, which are worth publishing provided that their validity is convincingly substantiated. Unfortunately, there are some doubts concerning this point.

% Explaining physics of computations’ results is not among the strengths of DNS. Accordingly, the authors do not attempt explaining physics of their findings. This is quite understandable and can be compensated by a convincing justification of the model assumptions and clear explanation of the model design. Unfortunately this is not the case with this paper. The main concerns are as follows:

% \textbf{1.} Equations (2) and (3) differ from standard formulation of the anelastic approximation (see, e.g., Sect.2.3 in Lantz and Fan 1999). Equation (2) combines magnetic pressure in a common term with gas pressure. This switches-off the magnetic buoyancy, which is essential for Tayler instability (figure 1 in Spruit 1999). Equation (3) replaces the diffusion term by $\tau$-relaxation. What is $\tau$ is not explained. Quotation of the origin and justification of the anelastic equations used in the paper is necessary.

% \textcolor{blue}{  The equations are different because EULAG solves the Lipps-Hemler (Journal of
% Atmospheric Sciences, v. 39, n. 10, p. 2192–2210, out. 1982) anelastic system of equations in its inviscid form. Viscosity, thermal conduction and magnetic diffusivity are accounted by MPDATA (Smolarkiewicz, P. K. , International Journal
% for Numerical Methods in Fluids, Wiley Online Library, v. 50, n. 10, p. 1123–1144, 2006). 
% The common term that engulfs both magnetic and gas pressure can be written as: $p^\prime = p^\prime_g + \frac{\boldsymbol{B}^2}{2\mu_0}$, where the terms are gas pressure and magnetic pressure, respectively. Thus, the magnetic pressure, and therefore magnetic buoyancy, are still accounted. The $p^\prime$ equation has been added to the main text, in the paragraph after Eq. 4. The term $\frac{\Theta^\prime}{\tau}$ does not replace the thermal diffusion. Note that $\Theta^\prime$ corresponds to perturbations around the ambient state. Thus, $\tau$ is a relaxation term that helps the implicit diffusion maintaining the mean equilibria of the system. 
% In this context, $\tau$ is the time scale for the perturbations to relax, and works in all scales of the system. A general discussion about this formulation can be found in (Cossete et al., ApJ, v. 841,
% n. 1, p. 65, maio 2017). We have also clarified this in the manuscript (see paragraph following Eq. 4).
% }

% \textbf{2.} The fluid layer of the model comprises the upper part of radiation zone but low part of unstable convection zone also. The change of the red line in Fig.1(b) to negative values in the upper part of the layer is not shown. Lines 49-50 in the right column of page 4 tell that stability is assumed for convection zone for simplicity. It is understandable that anelastic approximation demands deviations from adiabatic stratification to be small and the deviation is small inside the convection zone, but assuming the unstable convection zone to be stable “for simplicity” is strange. I encourage the authors to keep to the radiation zone. It is also possible to apply the anelastic approximation to a layer with strongly subadiabatic stratification (deep radiation zone) if the radial extend of the simulation layer is small.

% \textcolor{blue}{ 
% The study was not meant to reproduce the TI in the solar tachocline neither in the solar convection zone. We aimed to study the TI in a thin stable region, and used characteristic values similar to the lower part of the solar tachocline. We have altered the text in order to clarify this misunderstanding. Different setups of stratification were studied in Guerrero et al. (MNRAS, v. 490, n. 3,p. 4281–4291, Dec 201). In Fig.1(b) the negative values are not seen because the y-scale is logarithmic. The presence of the JCD model in Fig.1 is meant only as a comparison tool to help the reader visualize our model.
% % 
% % In Fig.1(b) the negative values are not seen as the y-scale is logarithmic. The referee is right that the later part of the graphic represent the lower part of the convection zone for the JCD model. In this sense the figure is misleading. The study was not meant to reproduce the TI in the solar tachocline neither in the solar convection zone. We aimed to study the TI in a thin stable region, and used characteristic values similar to the lower part of the solar tachocline. We have altered the text in order to clarify this misunderstanding. Different setups of stratification were studied in Guerrero et al. (MNRAS, v. 490, n. 3,p. 4281–4291, Dec 201)
% }

% \textbf{3.} The initial field of Eqs. (8) and (9) does not fit the top boundary condition. What does the perfect conductor bottom boundary condition mean for the equation with omitted magnetic diffusion is not clear.

% \textcolor{blue}{  The magnetic field radial profile, from Eqs. 8 and 9,  has a Gaussian profile. The standard deviation chosen in Eq. 9 results in a field intensity at the boundaries at the order of $10^{-3}$ and are set to zero at the by the top boundary condition. These value could be altered by a different standard deviation, though our choice is already low enough for practical purposes.
% %
% Inside the simulated region magnetic diffusion is not nonexistent, it is only delegated to the numerical scheme. What the boundary condition do is assume that, at the border, the magnetic diffusion will be much smaller than the effective turbulent diffusion.
% % 
% % The radial part of initial field goes to zero at both bottom and top boundaries, following Eq. 9. The latitudinal part of Eq. 8 does the same near the equator and the poles. Inside the simulated region magnetic diffusion is not nonexistent, it is only delegated to the numerical scheme. Such boundaries can be numerically enforced by setting the tangential components of the magnetic field to zero.
% }

% \textbf{4.} The origin of deviations from axial symmetry is unclear. How do the non-axisymmetric disturbances emerge? Lines 23, 24 in the right column of p.5 tell that it is unbalanced magnetic force of background field that imposes disturbances. The background state is axially symmetric. A substitution of the initial state in the equation system returns axially symmetric time derivatives. How does the numerical code decide at which longitudes deviations from axial symmetry should emerge from axially symmetric preceding state? This should be explained in the text.

% \textcolor{blue}{  To balance the introduction of the initial magnetic field $\Theta^\prime$ is increased. Although most of its energy is present in mode $m=0$, the other modes are also exited due to numerical noise (i.e. truncation and round-off errors). Despite having energy values compatible with numerical precision, the perturbations in higher modes are present through the simulation and sufficient to start TI. This evolution can be seen in the spectral movies added to the supplementary material. This explanation was also extended in the main text.
% }

% The paper can be reconsidered for publication after clarifying the items above.


% \scriptsize{
% % \bibliographystyle{abnt-alf}  % abnt-alf or abnt-num unsrt
% % %\bibliography{ref}
% \bibliography{references}
% }
% \end{document}









\input{preamble.tex} %Importando o preâmbulo

% ---------------------------------------------------------- 
% CONFIGURAÇÕES PESSOAIS
% ----------------------------------------------------------	
\newcommand{\soptitle}{Answer To Referee}
\newcommand{\yourname}{Guilherme Monteiro}
\newcommand{\youremail}{guiaudias@ufmg.br}

% ----------------------------------------------------------
\begin{document}
% ----------------------------------------------------------
%Making my own title
\begin{center}\LARGE\soptitle\\
\large \yourname\\\youremail\\ 
\end{center}
\hrule
\vspace{0.1cm}
\hrule height 0.1cm
\vspace{0.3cm}
% ----------------------------------------------------------

\section*{Comments to the Author}

The paper “Global simulations of Tayler instability in stellar interiors: a long-time multi-stage evolution of the magnetic field” by Guilherme Monteiro et al. studies Tayler instability of toroidal magnetic fields in stably stratified stellar interiors by 3D direct numerical simulations (DNS). The computations reproduce the formerly known initial exponential growth of the instability and discover new essentially nonlinear stages of saturation and eventual decay in the instability development. These are significant new results, which are worth publishing provided that their validity is convincingly substantiated. Unfortunately, there are some doubts concerning this point.

Explaining physics of computations’ results is not among the strengths of DNS. Accordingly, the authors do not attempt explaining physics of their findings. This is quite understandable and can be compensated by a convincing justification of the model assumptions and clear explanation of the model design. Unfortunately this is not the case with this paper.

\textcolor{blue}{We thank the Reviewer for the comments and
suggestions. In the revised manuscript, we accommodated all of them
in the letter or spirit. However, we wish to clarify up front that
the simulations presented in the paper are not DNS, as claimed by
the Reviewer, but ILES (for "implicit large eddy simulation") as
stated in the third paragraph of the right column on page 2 of the
paper. ILES is nowadays widely known and appreciated; cf. Cambridge
University Press monograph https://doi.org/10.1017/CBO9780511618604 .}

The main concerns are as follows:

\textbf{1.} Equations (2) and (3) differ from standard formulation of the anelastic approximation (see, e.g., Sect.2.3 in Lantz and Fan 1999). Equation (2) combines magnetic pressure in a common term with gas pressure. This switches-off the magnetic buoyancy, which is essential for Tayler instability (figure 1 in Spruit 1999). Equation (3) replaces the diffusion term by $\tau$-relaxation. What is $\tau$ is not explained. Quotation of the origin and justification of the anelastic equations used in the paper is necessary.

\textcolor{blue}{The governing anelastic equations of EULAG-MHD
adopt the Lipps-Hemler formulation (Lipps and Hamler, 1982; Lipps,
1990 --- both quoted in the revised paper), proven successful in
numerous applications to solar/stellar dynamics. Notably, the same
equations were used in our earlier MNRAS paper on the Tyler instability
(Guerrero et al, 2019a) referenced in the current work. These
equations, when optionally integrated in the inviscid form, delegate
dissipation, thermal conduction and magnetic diffusivity to truncation
terms of the non-oscillatory MPDATA (Smolarkiewicz, 2006), effecting
in the ILES property of the performed calculations. In turn, the
relaxation term $\frac{\Theta^\prime}{\tau}$ does not replace thermal
conduction but attenuates the potential temperature to the ambient
state, on the long time-scale $\tau$; for an extended discussion
see (Cossete et al., 2017), referenced in the paper.  Indeed, as noted by the Reviewer, 
the magnetic pressure is subsumed
with the thermodynamic pressure (Ghizaru et al, 2010; Smolarkiewicz and Charbonneau 2013;
Cosette et al, 2017; Guerrero et al, 2016, 2019a, 2019b --- all
quoted in the paper). To accomodate the Reviewer comment, the
narrative past Eqs.  (1)-(4) has been accordingly revised. }


\textbf{2.} The fluid layer of the model comprises the upper part of radiation zone but low part of unstable convection zone also. The change of the red line in Fig.1(b) to negative values in the upper part of the layer is not shown. Lines 49-50 in the right column of page 4 tell that stability is assumed for convection zone for simplicity. It is understandable that anelastic approximation demands deviations from adiabatic stratification to be small and the deviation is small inside the convection zone, but assuming the unstable convection zone to be stable “for simplicity” is strange. I encourage the authors to keep to the radiation zone. It is also possible to apply the anelastic approximation to a layer with strongly subadiabatic stratification (deep radiation zone) if the radial extend of the simulation layer is small.

\textcolor{blue}{ 
The study was not meant to reproduce the TI in the solar tachocline neither in the solar convection zone. We aimed to study the TI in a thin stable region, and used characteristic values similar to the lower part of the solar tachocline. We have altered the text in order to clarify this misunderstanding. Different setups of stratification were studied in Guerrero et al, 2019a, referenced in the current work. In Fig.1(b) the negative values are not seen because the y-scale is logarithmic. The presence of the JCD model in Fig.1 is meant only as a comparison tool to help the reader visualize our model.
% 
% In Fig.1(b) the negative values are not seen as the y-scale is logarithmic. The referee is right that the later part of the graphic represent the lower part of the convection zone for the JCD model. In this sense the figure is misleading. The study was not meant to reproduce the TI in the solar tachocline neither in the solar convection zone. We aimed to study the TI in a thin stable region, and used characteristic values similar to the lower part of the solar tachocline. We have altered the text in order to clarify this misunderstanding. Different setups of stratification were studied in Guerrero et al. (MNRAS, v. 490, n. 3,p. 4281–4291, Dec 201)
}

\textbf{3.} The initial field of Eqs. (8) and (9) does not fit the top boundary condition. What does the perfect conductor bottom boundary condition mean for the equation with omitted magnetic diffusion is not clear.

\textcolor{blue}{  The magnetic field radial profile, from Eqs. 8 and 9,  has a Gaussian profile. The standard deviation chosen in Eq. 9 results in a field intensity at the boundaries at the order of $10^{-3}$ and are set to zero at the by the top boundary condition. These value could be altered by a different standard deviation, though our choice is already low enough for practical purposes.
%
Inside the simulated region magnetic diffusion is not nonexistent, it is only delegated to the numerical scheme. What the boundary condition do is assume that, at the border, the magnetic diffusion will be much smaller than the effective turbulent diffusion.
% 
% The radial part of initial field goes to zero at both bottom and top boundaries, following Eq. 9. The latitudinal part of Eq. 8 does the same near the equator and the poles. Inside the simulated region magnetic diffusion is not nonexistent, it is only delegated to the numerical scheme. Such boundaries can be numerically enforced by setting the tangential components of the magnetic field to zero.
}

\textbf{4.} The origin of deviations from axial symmetry is unclear. How do the non-axisymmetric disturbances emerge? Lines 23, 24 in the right column of p.5 tell that it is unbalanced magnetic force of background field that imposes disturbances. The background state is axially symmetric. A substitution of the initial state in the equation system returns axially symmetric time derivatives. How does the numerical code decide at which longitudes deviations from axial symmetry should emerge from axially symmetric preceding state? This should be explained in the text.

\textcolor{blue}{  To balance the introduction of the initial magnetic field $\Theta^\prime$ is increased. Although most of its energy is present in mode $m=0$, the other modes are also excited due to numerical noise (i.e. truncation and round-off errors). Despite having energy values compatible with numerical precision, the perturbations in higher modes are present through the simulation and sufficient to start TI. This evolution can be seen in the spectral movies added to the supplementary material. This explanation was also extended in the main text.
}

The paper can be reconsidered for publication after clarifying the items above.



\scriptsize{
% \bibliographystyle{abnt-alf}  % abnt-alf or abnt-num unsrt
% %\bibliography{ref}
% \bibliography{references}
}
\end{document}
